MAG: Multi-Modal Aligned Autoregressive Co-Speech Gesture Generation without Vector Quantization

This work focuses on full-body co-speech gesture generation. Existing methods typically employ an autoregressive model accompanied by vector-quantized tokens for gesture generation, which results in information loss and compromises the realism of the generated gestures. To address this, inspired by the natural continuity of real-world human motion, we propose MAG, a novel multi-modal aligned framework for high-quality and diverse co-speech gesture synthesis without relying on discrete tokenization. Specifically, (1) we introduce a motion-text-audio-aligned variational autoencoder (MTA-VAE), which leverages pre-trained WavCaps' text and audio embeddings to enhance both semantic and rhythmic alignment with motion, ultimately producing more realistic gestures. (2) Building on this, we propose a multimodal masked autoregressive model (MMAG) that enables autoregressive modeling in continuous motion embeddings through diffusion without vector quantization. To further ensure multi-modal consistency, MMAG incorporates a hybrid granularity audio-text fusion block, which serves as conditioning for diffusion process. Extensive experiments on two benchmark datasets demonstrate that MAG achieves stateof-the-art performance both quantitatively and qualitatively, producing highly realistic and diverse co-speech gestures.The code will be released to facilitate future research.

==> _constants.tex <==
\def\cvprPaperID{6138}
\def\confName{ICCV}
\def\confYear{2025}

% other names are also welcome.
%\def\paperTitle{MarDGesture: Masked Autoregressive Diffusion for Gesture Generation}
\def\paperTitle{MarDGesture: Autoregressive Gesture Generation without Vector Quantization}
% \def\paperTitle{LivelySpeaker: Semantic and Rhythm-aware Co-Speech Gesture Generation}

\def\authorBlock{
    Binjie Liu\textsuperscript{\rm 1,}\thanks{Equal contribution} \quad
 \\ \\
    \textsuperscript{\rm 1}Communication University of China \quad
    % {\tt\small \{binjieliu\}@binjieliu@cuc.edu.cn \qua\\
    % {\tt \small xi.shen@enpc.fr \quad wen.guo@inria.fr}\\
    \\
    \url{https://github.com/lovemino/margesture}
}


% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


\newcommand{\xl}[1]{{\color{black}#1}}
\newcommand{\xlc}[1]{{\color{orange}#1}}


\newcommand{\ra}{\textcolor{red}{\textbf{R1}}}
\newcommand{\rb}{\textcolor{orange}{\textbf{R2}}}
\newcommand{\rc}{\textcolor{blue}{\textbf{R3}}}



==> _macros.tex <==
%% PACKAGES (also see cvpr_header.tex)

\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage[table,xcdraw]{xcolor}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{xcolor}

\usepackage{amsmath}

\usepackage[hang,flushmargin]{footmisc}

% Unfortunately, this package interferes with arxiv's stamp
\ifcamera \usepackage[accsupp]{axessibility} \fi

%% MACROS

% \newcommand{\authorname}[1]{{\textcolor{blue}{[Author: #1]}}}
% ...

% \newcommand{\commandname}{string\xspace}
% \definecolor{colorname}{rgb}{0.92,0.49,0.19}

\newcommand{\xiaodong}[1]{{\textcolor{blue}{[Xiaodong: #1]}}}
\newcommand{\sx}[1]{{\textcolor{purple}{[Xi: #1]}}}
\newcommand{\wen}[1]{{\textcolor{teal}{[Wen: #1]}}}

\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
\ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

% Reviewer commands (1 to 5), e.g. \R{1}, \R{2}
\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor[rgb]{1,0.33,0.2}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor[rgb]{0.2,0.7,0.1}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{cyan}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}


==> cvpr_header.tex <==
\ifreview \usepackage[review]{cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{cvpr} \fi
\ifcamera \usepackage{cvpr} \fi

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}

\input{_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%


\usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table.}{Tables}
\crefname{figure}{Fig.}{Figs.}


% General
\hypersetup{
    colorlinks = true,
    linkbordercolor = {white},
    % <your other options...>,
    citecolor=blue,
    urlcolor=magenta
}

\frenchspacing


==> figures/distribution.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ted_distribution_hf.pdf}
    \vspace{-2em}
    \caption{We plot the $L_2$ loss histogram on the training samples of the pre-trained trimodal method~\cite{trimodal}. Although it is learned from multiple conditions~(\eg, text, audio), their methods are still dominated by repeated rhythm, and hard to model the rarely appeared diversity gestures, \eg, the semantic-aware motions.}
    \label{fig:distribution}
\end{figure}

==> figures/teaser.tex <==
\twocolumn[{
\maketitle
\begin{center}
    \captionsetup{type=figure}
    \includegraphics[width=1.\linewidth]{figures/teaser.png}
    \vspace{-1.em}
    \captionof{figure}{
    We propose xxx, a novel system that
    % first stage is a  which enables text-controllable semantic-aware gesture generation. While SAG can generate semantic meaningful gestures, it often fails to align the generated gestures with the rhythm, which limits the realism of the generated motion. To solve this problem, we propose a  as the second stage of the framework which can align the generated motion to the input speech. By combining these two stages, our proposed method can generate gestures with semantic awareness while synchronizing closely with the input speech. 
    % \xiaodong{need check: x-aware or x-Aware (make it consistent in overall paper), Do we need to highlight the SAG+RAG pipeline?}
    % done 正文部分rhythm semantic-aware generator
    % 图 标题Rhythm Semantic-aware
    }
    \label{fig:First}
\end{center}
}]

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> math_utils.tex <==
% define all math-related symbols as global commands here

\newcommand{\exemplar}{ E }
